Lyapunov Event-triggered Stabilization with a Known Convergence Rate

A constructive tool of nonlinear control systems design, the method of Control Lyapunov Functions (CLF) has found numerous applications in stabilization problems for continuous time, discrete-time and hybrid systems. In this paper, we address the fundamental question: given a CLF, corresponding to the continuous-time controller with some predefined (e.g. exponential) convergence rate, can the same convergence rate be provided by an event-triggered controller? Under certain assumptions, we give an affirmative answer to this question and show that the corresponding event-based controllers provide positive dwelltimes between the consecutive events. Furthermore, we prove the existence of self-triggered and periodic event-triggered controllers, providing stabilization with a known convergence rate.

==> 4periodic.tex <==
\section{Self-triggered and periodic event-triggered stabilization} 

One may notice that the dwell-time estimates, obtained in Section~\ref{sec.event}, employ the functions $\vk(\cdot)$ and $\nu(\cdot)$ from Assumptions~\ref{ass.F} and~\ref{ass.gradient} and $M(\cdot)$ from~\eqref{eq.non-degen1}. Essentially, we need only
